Velocity Gradients: Magnetic Field Tomography towards the Supernova Remnant W44

As a novel approach for tracing interstellar magnetic fields, the Velocity Gradient Technique (VGT) has been proven to be effective for probing magnetic fields in the diffuse interstellar medium (ISM). In this work, we verify the VGT in a broader context by applying the technique to a molecular cloud interacting with the supernovae remnant (SNR) W44. We probe the magnetic fields with the VGT using CO, $\rm HCO^+$, and H I emission lines and make a comparison with the Planck 353 GHZ dust polarization. We show that the VGT gives an accurate measurement that coheres with the Planck polarization especially in intense molecular gas emission regions. We further study the foreground's contribution to the polarization that results in a misalignment between the VGT and the Planck measurements in low-intensity molecular gas areas. We advance the VGT to achieve magnetic field tomography by decomposing the W44 into various velocity components. We show that W44's velocity component at $v\sim45$ km s$^{-1}$ exhibits the largest coverage and gives the best agreement with Planck polarization in terms of magnetic field orientation.

==> reference <==
@ARTICLE{2018AJ....156..123A,
       author = {{Astropy Collaboration} and {Price-Whelan}, A.~M. and {Sip{\H{o}}cz}, B.~M. and {G{\"u}nther}, H.~M. and {Lim}, P.~L. and {Crawford}, S.~M. and {Conseil}, S. and {Shupe}, D.~L. and {Craig}, M.~W. and {Dencheva}, N. and {Ginsburg}, A. and {VanderPlas}, J.~T. and {Bradley}, L.~D. and {P{\'e}rez-Su{\'a}rez}, D. and {de Val-Borro}, M. and {Aldcroft}, T.~L. and {Cruz}, K.~L. and {Robitaille}, T.~P. and {Tollerud}, E.~J. and {Ardelean}, C. and {Babej}, T. and {Bach}, Y.~P. and {Bachetti}, M. and {Bakanov}, A.~V. and {Bamford}, S.~P. and {Barentsen}, G. and {Barmby}, P. and {Baumbach}, A. and {Berry}, K.~L. and {Biscani}, F. and {Boquien}, M. and {Bostroem}, K.~A. and {Bouma}, L.~G. and {Brammer}, G.~B. and {Bray}, E.~M. and {Breytenbach}, H. and {Buddelmeijer}, H. and {Burke}, D.~J. and {Calderone}, G. and {Cano Rodr{\'\i}guez}, J.~L. and {Cara}, M. and {Cardoso}, J.~V.~M. and {Cheedella}, S. and {Copin}, Y. and {Corrales}, L. and {Crichton}, D. and {D'Avella}, D. and {Deil}, C. and {Depagne}, {\'E}. and {Dietrich}, J.~P. and {Donath}, A. and {Droettboom}, M. and {Earl}, N. and {Erben}, T. and {Fabbro}, S. and {Ferreira}, L.~A. and {Finethy}, T. and {Fox}, R.~T. and {Garrison}, L.~H. and {Gibbons}, S.~L.~J. and {Goldstein}, D.~A. and {Gommers}, R. and {Greco}, J.~P. and {Greenfield}, P. and {Groener}, A.~M. and {Grollier}, F. and {Hagen}, A. and {Hirst}, P. and {Homeier}, D. and {Horton}, A.~J. and {Hosseinzadeh}, G. and {Hu}, L. and {Hunkeler}, J.~S. and {Ivezi{\'c}}, {\v{Z}}. and {Jain}, A. and {Jenness}, T. and {Kanarek}, G. and {Kendrew}, S. and {Kern}, N.~S. and {Kerzendorf}, W.~E. and {Khvalko}, A. and {King}, J. and {Kirkby}, D. and {Kulkarni}, A.~M. and {Kumar}, A. and {Lee}, A. and {Lenz}, D. and {Littlefair}, S.~P. and {Ma}, Z. and {Macleod}, D.~M. and {Mastropietro}, M. and {McCully}, C. and {Montagnac}, S. and {Morris}, B.~M. and {Mueller}, M. and {Mumford}, S.~J. and {Muna}, D. and {Murphy}, N.~A. and {Nelson}, S. and {Nguyen}, G.~H. and {Ninan}, J.~P. and {N{\"o}the}, M. and {Ogaz}, S. and {Oh}, S. and {Parejko}, J.~K. and {Parley}, N. and {Pascual}, S. and {Patil}, R. and {Patil}, A.~A. and {Plunkett}, A.~L. and {Prochaska}, J.~X. and {Rastogi}, T. and {Reddy Janga}, V. and {Sabater}, J. and {Sakurikar}, P. and {Seifert}, M. and {Sherbert}, L.~E. and {Sherwood-Taylor}, H. and {Shih}, A.~Y. and {Sick}, J. and {Silbiger}, M.~T. and {Singanamalla}, S. and {Singer}, L.~P. and {Sladen}, P.~H. and {Sooley}, K.~A. and {Sornarajah}, S. and {Streicher}, O. and {Teuben}, P. and {Thomas}, S.~W. and {Tremblay}, G.~R. and {Turner}, J.~E.~H. and {Terr{\'o}n}, V. and {van Kerkwijk}, M.~H. and {de la Vega}, A. and {Watkins}, L.~L. and {Weaver}, B.~A. and {Whitmore}, J.~B. and {Woillez}, J. and {Zabalza}, V. and {Astropy Contributors}},
        title = "{The Astropy Project: Building an Open-science Project and Status of the v2.0 Core Package}",
      journal = {\aj},
     keywords = {methods: data analysis, methods: miscellaneous, methods: statistical, reference systems, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = sep,
       volume = {156},
       number = {3},
          eid = {123},
        pages = {123},
          doi = {10.3847/1538-3881/aabc4f},
archivePrefix = {arXiv},
       eprint = {1801.02634},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..123A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJS..216....2A,
       author = {{Andersson}, M. and {Grumer}, J. and {Ryde}, N. and {Blackwell-Whitehead}, R. and {Hutton}, R. and {Zou}, Y. and {J{\"o}nsson}, P. and {Brage}, T.},
        title = "{Hyperfine-dependent gf-values of Mn I Lines in the 1.49-1.80 {\ensuremath{\mu}}m H Band}",
      journal = {\apjs},
     keywords = {atomic data, infrared: stars, line: identification, methods: laboratory: atomic, methods: numerical, stars: abundances, Astrophysics - Solar and Stellar Astrophysics, Physics - Atomic Physics},
         year = 2015,
        month = jan,
       volume = {216},
       number = {1},
          eid = {2},
        pages = {2},
          doi = {10.1088/0067-0049/216/1/2},
archivePrefix = {arXiv},
       eprint = {1406.2942},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..216....2A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2013A&A...558A..33A,
       author = {{Astropy Collaboration} and {Robitaille}, Thomas P. and
         {Tollerud}, Erik J. and {Greenfield}, Perry and {Droettboom}, Michael and
         {Bray}, Erik and {Aldcroft}, Tom and {Davis}, Matt and
         {Ginsburg}, Adam and {Price-Whelan}, Adrian M. and
         {Kerzendorf}, Wolfgang E. and {Conley}, Alexander and {Crighton}, Neil and
         {Barbary}, Kyle and {Muna}, Demitri and {Ferguson}, Henry and
         {Grollier}, Fr{\'e}d{\'e}ric and {Parikh}, Madhura M. and
         {Nair}, Prasanth H. and {Unther}, Hans M. and {Deil}, Christoph and
         {Woillez}, Julien and {Conseil}, Simon and {Kramer}, Roban and
         {Turner}, James E.~H. and {Singer}, Leo and {Fox}, Ryan and
         {Weaver}, Benjamin A. and {Zabalza}, Victor and {Edwards}, Zachary I. and
         {Azalee Bostroem}, K. and {Burke}, D.~J. and {Casey}, Andrew R. and
         {Crawford}, Steven M. and {Dencheva}, Nadia and {Ely}, Justin and
         {Jenness}, Tim and {Labrie}, Kathleen and {Lim}, Pey Lian and
         {Pierfederici}, Francesco and {Pontzen}, Andrew and {Ptak}, Andy and
         {Refsdal}, Brian and {Servillat}, Mathieu and {Streicher}, Ole},
        title = "{Astropy: A community Python package for astronomy}",
      journal = {\aap},
     keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2013",
        month = "Oct",
       volume = {558},
          eid = {A33},
        pages = {A33},
          doi = {10.1051/0004-6361/201322068},
archivePrefix = {arXiv},
       eprint = {1307.6212},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...558A..33A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996A&AS..117..393B,
       author = {{Bertin}, E. and {Arnouts}, S.},
        title = "{SExtractor: Software for source extraction.}",
      journal = {\aaps},
     keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
         year = "1996",
        month = "Jun",
       volume = {117},
        pages = {393-404},
          doi = {10.1051/aas:1996164},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&AS..117..393B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018AJ....156...82C,
       author = {{Cloutier}, Ryan and {Doyon}, Ren{\'e} and {Bouchy}, Francois and
         {H{\'e}brard}, Guillaume},
        title = "{Quantifying the Observational Effort Required for the Radial Velocity Characterization of TESS Planets}",
      journal = {\aj},
     keywords = {methods: analytical, planets and satellites: detection, planets and satellites: fundamental parameters, techniques: radial velocities, Astrophysics - Earth and Planetary Astrophysics},
         year = "2018",
        month = "Aug",
       volume = {156},
       number = {2},
          eid = {82},
        pages = {82},
          doi = {10.3847/1538-3881/aacea9},
archivePrefix = {arXiv},
       eprint = {1807.01263},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156...82C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014A&A...565A..74C,
       author = {{Cardillo}, M. and {Tavani}, M. and {Giuliani}, A. and {Yoshiike}, S. and {Sano}, H. and {Fukuda}, T. and {Fukui}, Y. and {Castelletti}, G. and {Dubner}, G.},
        title = "{The supernova remnant W44: Confirmations and challenges for cosmic-ray acceleration}",
      journal = {\aap},
     keywords = {acceleration of particles, astroparticle physics, shock waves, radiation mechanisms: non-thermal, ISM: supernova remnants, gamma rays: ISM, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = may,
       volume = {565},
          eid = {A74},
        pages = {A74},
          doi = {10.1051/0004-6361/201322685},
archivePrefix = {arXiv},
       eprint = {1403.1250},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...565A..74C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009MNRAS.400.2050G,
       author = {{G{\"u}ver}, Tolga and {{\"O}zel}, Feryal},
        title = "{The relation between optical extinction and hydrogen column density in the Galaxy}",
      journal = {\mnras},
     keywords = {dust, extinction, supernova remnants, X-rays: ISM, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2009,
        month = dec,
       volume = {400},
       number = {4},
        pages = {2050-2053},
          doi = {10.1111/j.1365-2966.2009.15598.x},
archivePrefix = {arXiv},
       eprint = {0903.2057},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.400.2050G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2008AA...487..993K,
       author = {{Kauffmann}, J. and {Bertoldi}, F. and {Bourke}, T.~L. and {Evans}, N.~J., II and {Lee}, C.~W.},
        title = "{MAMBO mapping of Spitzer c2d small clouds and cores}",
      journal = {\aap},
     keywords = {stars: formation, ISM: evolution, ISM: structure, ISM: dust, extinction, ISM: clouds, Astrophysics},
         year = 2008,
        month = sep,
       volume = {487},
       number = {3},
        pages = {993-1017},
          doi = {10.1051/0004-6361:200809481},
archivePrefix = {arXiv},
       eprint = {0805.4205},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...487..993K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2011ApJ...742L..30G,
       author = {{Giuliani}, A. and {Cardillo}, M. and {Tavani}, M. and {Fukui}, Y. and {Yoshiike}, S. and {Torii}, K. and {Dubner}, G. and {Castelletti}, G. and {Barbiellini}, G. and {Bulgarelli}, A. and {Caraveo}, P. and {Costa}, E. and {Cattaneo}, P.~W. and {Chen}, A. and {Contessi}, T. and {Del Monte}, E. and {Donnarumma}, I. and {Evangelista}, Y. and {Feroci}, M. and {Gianotti}, F. and {Lazzarotto}, F. and {Lucarelli}, F. and {Longo}, F. and {Marisaldi}, M. and {Mereghetti}, S. and {Pacciani}, L. and {Pellizzoni}, A. and {Piano}, G. and {Picozza}, P. and {Pittori}, C. and {Pucella}, G. and {Rapisarda}, M. and {Rappoldi}, A. and {Sabatini}, S. and {Soffitta}, P. and {Striani}, E. and {Trifoglio}, M. and {Trois}, A. and {Vercellone}, S. and {Verrecchia}, F. and {Vittorini}, V. and {Colafrancesco}, S. and {Giommi}, P. and {Bignami}, G.},
        title = "{Neutral Pion Emission from Accelerated Protons in the Supernova Remnant W44}",
      journal = {\apjl},
     keywords = {acceleration of particles, cosmic rays, gamma rays: general, ISM: supernova remnants, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2011,
        month = dec,
       volume = {742},
       number = {2},
          eid = {L30},
        pages = {L30},
          doi = {10.1088/2041-8205/742/2/L30},
archivePrefix = {arXiv},
       eprint = {1111.4868},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...742L..30G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015yCat..22160002A,
       author = {{Andersson}, M. and {Grumer}, J. and {Ryde}, N. and {Blackwell-Whitehead}, R. and {Hutton}, R. and {Zou}, Y. and {Jonsson}, P. and {Brage}, T.},
        title = "{VizieR Online Data Catalog: MnI hyperfine lines in the 1.4-1.8um (H) band (Andersson+, 2015)}",
      journal = {VizieR Online Data Catalog},
     keywords = {Atomic physics, Line Profiles, Spectra: infrared},
         year = 2015,
        month = feb,
          eid = {J/ApJS/216/2},
        pages = {J/ApJS/216/2},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015yCat..22160002A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...503..827X,
       author = {{Xiao}, L. and {Reich}, W. and {F{\"u}rst}, E. and {Han}, J.~L.},
        title = "{Radio properties of the low surface brightness SNR G65.2+5.7}",
      journal = {\aap},
     keywords = {ISM: supernova remnants, ISM: magnetic fields, radio continuum: ISM, radiation mechanisms: non-thermal, Astrophysics - Astrophysics of Galaxies},
         year = 2009,
        month = sep,
       volume = {503},
       number = {3},
        pages = {827-836},
          doi = {10.1051/0004-6361/200911706},
archivePrefix = {arXiv},
       eprint = {0904.3170},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...503..827X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008A&A...482..783X,
       author = {{Xiao}, L. and {F{\"u}rst}, E. and {Reich}, W. and {Han}, J.~L.},
        title = "{Radio spectral properties and the magnetic field of the SNR S147}",
      journal = {\aap},
     keywords = {ISM: supernova remnants, radio continuum: ISM, techniques: polarimetric, Astrophysics},
         year = 2008,
        month = may,
       volume = {482},
       number = {3},
        pages = {783-792},
          doi = {10.1051/0004-6361:20078461},
archivePrefix = {arXiv},
       eprint = {0801.4803},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...482..783X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005AdSpR..35.1707K,
       author = {{Krucker}, S{\"a}m and {Fivian}, M.~D. and {Lin}, R.~P.},
        title = "{Hard X-ray footpoint motions in solar flares: Comparing magnetic reconnection models with observations}",
      journal = {Advances in Space Research},
         year = 2005,
        month = jan,
       volume = {35},
       number = {10},
        pages = {1707-1711},
          doi = {10.1016/j.asr.2005.05.054},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005AdSpR..35.1707K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2018ApJ...853...96L,
       author = {{Lazarian}, A. and {Yuen}, Ka Ho},
        title = "{Tracing Magnetic Fields with Spectroscopic Channel Maps}",
      journal = {\apj},
     keywords = {ISM: magnetic fields, ISM: structure, Astrophysics - Astrophysics of Galaxies},
         year = "2018b",
        month = jan,
       volume = {853},
       number = {1},
          eid = {96},
        pages = {96},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...853...96L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...805...23C,
       author = {{Corrales}, Lia},
        title = "{X-Ray Scattering Echoes and Ghost Halos from the Intergalactic Medium: Relation to the Nature of AGN Variability}",
      journal = {\apj},
     keywords = {accretion, accretion disks, dust, extinction, quasars: general, intergalactic medium, X-rays: ISM, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = "2015",
        month = "May",
       volume = {805},
       number = {1},
          eid = {23},
        pages = {23},
          doi = {10.1088/0004-637X/805/1/23},
archivePrefix = {arXiv},
       eprint = {1503.01475},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...805...23C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013RMxAA..49..137F,
       author = {{Ferland}, G.~J. and {Porter}, R.~L. and {van Hoof}, P.~A.~M. and
         {Williams}, R.~J.~R. and {Abel}, N.~P. and {Lykins}, M.~L. and
         {Shaw}, G. and {Henney}, W.~J. and {Stancil}, P.~C.},
        title = "{The 2013 Release of Cloudy}",
      journal = {\rmxaa},
     keywords = {atomic processes, galaxies: active, methods: numerical, molecular processes, radiation mechanisms: general, Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2013",
        month = "Apr",
       volume = {49},
        pages = {137-163},
archivePrefix = {arXiv},
       eprint = {1302.4485},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013RMxAA..49..137F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1989BAAS...21..780H,
       author = {{Hanisch}, R.~J. and {Biemesderfer}, C.~D.},
        title = "{T$_{E}$X and LAT$_{E}$X Macro Definition Files for Astronomical Publications}",
    booktitle = {\baas},
         year = "1989",
        month = "Mar",
        pages = {780},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989BAAS...21..780H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{lamport94,
       author = {{Lamport}, L.},
        title = "{LaTeX: A Document Preparation System}",
    publisher = {Addison-Wesley Professional},
	 year = "1994",
      edition = {2},
	 isbn = {0201529831}
}

@ARTICLE{2017ApJ...837L..24Y,
       author = {{Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Tracing Interstellar Magnetic Field Using Velocity Gradient Technique: Application to Atomic Hydrogen Data}",
      journal = {\apjl},
     keywords = {ISM: general, ISM: magnetic fields, ISM: structure, magnetohydrodynamics: MHD, radio lines: ISM, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2017",
        month = mar,
       volume = {837},
       number = {2},
          eid = {L24},
        pages = {L24},
          doi = {10.3847/2041-8213/aa6255},
archivePrefix = {arXiv},
       eprint = {1701.07944},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...837L..24Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020arXiv200715344A,
       author = {{Alina}, D. and {Montillaud}, J. and {Hu}, Y. and {Lazarian}, A. and {Ristorcelli}, I. and {Abdikamalov}, E. and {Sagynbayeva}, S. and {Juvela}, M. and {Liu}, T. and {Carri{\`e}re}, J. -S.},
        title = "{Large-scale magnetic field in the Monoceros OB-1 East molecular cloud}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jul,
          eid = {arXiv:2007.15344},
        pages = {arXiv:2007.15344},
archivePrefix = {arXiv},
       eprint = {2007.15344},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200715344A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2019ApJ...874...25G,
       author = {{Gonz{\'a}lez-Casanova}, Diego F. and {Lazarian}, A.},
        title = "{Mapping of the Structure of the Galactic Magnetic Field with Velocity Gradients: Test Using Star Light Polarization}",
      journal = {\apj},
     keywords = {ISM: kinematics and dynamics, ISM: magnetic fields, methods: observational, turbulence, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = mar,
       volume = {874},
       number = {1},
          eid = {25},
        pages = {25},
          doi = {10.3847/1538-4357/ab0552},
archivePrefix = {arXiv},
       eprint = {1805.10329},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...874...25G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020MNRAS.496.2868L,
       author = {{Lu}, Zekun and {Lazarian}, A. and {Pogosyan}, Dmitri},
        title = "{Producing synthetic maps of dust polarization using a velocity channel gradient technique}",
      journal = {\mnras},
     keywords = {radio lines: ISM, ISM: magnetic fields, polarization, Diffuse radiation, ISM: structure, turbulence, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = aug,
       volume = {496},
       number = {3},
        pages = {2868-2884},
          doi = {10.1093/mnras/staa1570},
archivePrefix = {arXiv},
       eprint = {1910.02226},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.496.2868L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019NatAs...3..776H,
       author = {{Hu}, Yue and {Yuen}, Ka Ho and {Lazarian}, Victor and {Ho}, Ka Wai and {Benjamin}, Robert A. and {Hill}, Alex S. and {Lockman}, Felix J. and {Goldsmith}, Paul F. and {Lazarian}, Alex},
        title = "{Magnetic field morphology in interstellar clouds with the velocity gradient technique}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jun,
       volume = {3},
        pages = {776-782},
          doi = {10.1038/s41550-019-0769-0},
archivePrefix = {arXiv},
       eprint = {2002.09948},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019NatAs...3..776H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2019ApJ...884..137H,
       author = {{Hu}, Yue and {Yuen}, Ka Ho and {Lazarian}, A. and {Fissel}, Laura M. and {Jones}, P.~A. and {Cunningham}, M.~R.},
        title = "{Tracing Multi-scale Magnetic Field Structure Using Multiple Chemical Tracers in Giant Molecular Clouds}",
      journal = {\apj},
     keywords = {ISM: general, ISM: structure, radio lines: ISM, turbulence, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = oct,
       volume = {884},
       number = {2},
          eid = {137},
        pages = {137},
          doi = {10.3847/1538-4357/ab41f2},
archivePrefix = {arXiv},
       eprint = {1904.04391},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...884..137H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2020ApJ...888...96H,
       author = {{Hu}, Yue and {Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Predictions of Cosmic Microwave Background Foreground Dust Polarization Using Velocity Gradients}",
      journal = {\apj},
     keywords = {845, 847, 322, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2020",
        month = jan,
       volume = {888},
       number = {2},
          eid = {96},
        pages = {96},
          doi = {10.3847/1538-4357/ab60a5},
archivePrefix = {arXiv},
       eprint = {1910.05637},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...888...96H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021arXiv210503605H,
       author = {{Hu}, Yue and {Lazarian}, A. and {Wang}, Q. Daniel},
        title = "{Multi-scale Magnetic Fields in the Central Molecular Zone: Inference from the Gradient Technique}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = "2021",
        month = may,
          eid = {arXiv:2105.03605},
        pages = {arXiv:2105.03605},
archivePrefix = {arXiv},
       eprint = {2105.03605},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210503605H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...537..720L,
       author = {{Lazarian}, A. and {Pogosyan}, D.},
        title = "{Velocity Modification of H I Power Spectrum}",
      journal = {\apj},
     keywords = {Galaxy: Structure, ISM: Kinematics and Dynamics, Radio Lines: ISM, Astrophysics},
         year = 2000,
        month = jul,
       volume = {537},
       number = {2},
        pages = {720-748},
          doi = {10.1086/309040},
archivePrefix = {arXiv},
       eprint = {astro-ph/9901241},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...537..720L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ARA&A..53..501A,
       author = {{Andersson}, B. -G. and {Lazarian}, A. and {Vaillancourt}, John E.},
        title = "{Interstellar Dust Grain Alignment}",
      journal = {\araa},
         year = 2015,
        month = aug,
       volume = {53},
        pages = {501-539},
          doi = {10.1146/annurev-astro-082214-122414},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ARA&A..53..501A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020ApJ...898...65Y,
       author = {{Yuen}, Ka Ho and {Lazarian}, Alex},
        title = "{Advancing the Velocity Gradient Technique: Using Gradient Amplitudes and Handling Thermal Broadening}",
      journal = {\apj},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839},
         year = 2020,
        month = jul,
       volume = {898},
       number = {1},
          eid = {65},
        pages = {65},
          doi = {10.3847/1538-4357/ab9307},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...898...65Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ApJ...865...46L,
       author = {{Lazarian}, A. and {Yuen}, Ka Ho and {Ho}, Ka Wai and {Chen}, Junda and {Lazarian}, Victor and {Lu}, Zekun and {Yang}, Bo and {Hu}, Yue},
        title = "{Distribution of Velocity Gradient Orientations: Mapping Magnetization with the Velocity Gradient Technique}",
      journal = {\apj},
     keywords = {ISM: general, ISM: structure, magnetohydrodynamics: MHD, radio continuum: ISM, turbulence, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = sep,
       volume = {865},
       number = {1},
          eid = {46},
        pages = {46},
          doi = {10.3847/1538-4357/aad7ff},
archivePrefix = {arXiv},
       eprint = {1802.02984},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...865...46L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...784...38L,
       author = {{Lazarian}, A. and {Yan}, Huirong},
        title = "{Superdiffusion of Cosmic Rays: Implications for Cosmic Ray Acceleration}",
      journal = {\apj},
     keywords = {acceleration of particles, cosmic rays, galaxies: magnetic fields, magnetohydrodynamics: MHD, turbulence, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Earth and Planetary Astrophysics},
         year = 2014,
        month = mar,
       volume = {784},
       number = {1},
          eid = {38},
        pages = {38},
          doi = {10.1088/0004-637X/784/1/38},
archivePrefix = {arXiv},
       eprint = {1308.3244},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...784...38L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002PhRvL..89B1102Y,
       author = {{Yan}, Huirong and {Lazarian}, A.},
        title = "{Scattering of Cosmic Rays by Magnetohydrodynamic Interstellar Turbulence}",
      journal = {\prl},
     keywords = {98.70.Sa, 52.30.-q, 52.35.Ra, 95.30.Qd, Cosmic rays, Plasma dynamics and flow, Plasma turbulence, Magnetohydrodynamics and plasmas, Astrophysics},
         year = 2002,
        month = dec,
       volume = {89},
       number = {28},
          eid = {281102},
        pages = {281102},
          doi = {10.1103/PhysRevLett.89.281102},
archivePrefix = {arXiv},
       eprint = {astro-ph/0205285},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002PhRvL..89B1102Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...614..757Y,
       author = {{Yan}, Huirong and {Lazarian}, A.},
        title = "{Cosmic-Ray Scattering and Streaming in Compressible Magnetohydrodynamic Turbulence}",
      journal = {\apj},
     keywords = {Acceleration of Particles, ISM: Cosmic Rays, ISM: Magnetic Fields, Magnetohydrodynamics: MHD, Scattering, Turbulence, Astrophysics},
         year = 2004,
        month = oct,
       volume = {614},
       number = {2},
        pages = {757-769},
          doi = {10.1086/423733},
archivePrefix = {arXiv},
       eprint = {astro-ph/0408172},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...614..757Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008ApJ...673..942Y,
       author = {{Yan}, Huirong and {Lazarian}, A.},
        title = "{Cosmic-Ray Propagation: Nonlinear Diffusion Parallel and Perpendicular to Mean Magnetic Field}",
      journal = {\apj},
     keywords = {acceleration of particles, cosmic rays, ISM: magnetic fields, MHD, scattering, turbulence, Astrophysics},
         year = 2008,
        month = feb,
       volume = {673},
       number = {2},
        pages = {942-953},
          doi = {10.1086/524771},
archivePrefix = {arXiv},
       eprint = {0710.2617},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...673..942Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...779..140X,
       author = {{Xu}, Siyao and {Yan}, Huirong},
        title = "{Cosmic-Ray Parallel and Perpendicular Transport in Turbulent Magnetic Fields}",
      journal = {\apj},
     keywords = {cosmic rays, diffusion, magnetohydrodynamics: MHD, turbulence, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = dec,
       volume = {779},
       number = {2},
          eid = {140},
        pages = {140},
          doi = {10.1088/0004-637X/779/2/140},
archivePrefix = {arXiv},
       eprint = {1307.1346},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...779..140X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2013ApJ...774...10S,
       author = {{Sashida}, Tomoro and {Oka}, Tomoharu and {Tanaka}, Kunihiko and {Aono}, Kazuya and {Matsumura}, Shinji and {Nagai}, Makoto and {Seta}, Masumichi},
        title = "{Kinematics of Shocked Molecular Gas Adjacent to the Supernova Remnant W44}",
      journal = {\apj},
     keywords = {ISM: clouds, ISM: kinematics and dynamics, ISM: molecules, ISM: supernova remnants, radio lines: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = sep,
       volume = {774},
       number = {1},
          eid = {10},
        pages = {10},
          doi = {10.1088/0004-637X/774/1/10},
archivePrefix = {arXiv},
       eprint = {1307.6276},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...774...10S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1985MNRAS.217...99S,
       author = {{Smith}, A. and {Jones}, L.~R. and {Watson}, M.~G. and {Willingale}, R. and {Wood}, N. and {Seward}, F.~D.},
        title = "{X-ray observations of the supernova remnant W 44.}",
      journal = {\mnras},
     keywords = {Astronomical Models, Radio Sources (Astronomy), Supernova Remnants, X Ray Sources, Heao 2, Interstellar Matter, Molecular Clouds, Plasma Temperature, X Ray Spectra, Astronomy},
         year = 1985,
        month = nov,
       volume = {217},
        pages = {99-104},
          doi = {10.1093/mnras/217.1.99},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985MNRAS.217...99S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997ApJ...488..781H,
       author = {{Harrus}, Ilana M. and {Hughes}, John P. and {Singh}, K.~P. and {Koyama}, K. and {Asaoka}, I.},
        title = "{Interpretation of the Center-filled Emission from the Supernova Remnant W44}",
      journal = {\apj},
     keywords = {ISM: Abundances, ISM: individual (W44) -- nuclear reactions, nucleosynthesis, abundances, shock waves -- supernova remnants, X-Rays: ISM, Astrophysics},
         year = 1997,
        month = oct,
       volume = {488},
       number = {2},
        pages = {781-791},
          doi = {10.1086/304717},
archivePrefix = {arXiv},
       eprint = {astro-ph/9705239},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...488..781H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ApJS..234....2P,
       author = {{Peek}, J.~E.~G. and {Babler}, Brian L. and {Zheng}, Yong and {Clark}, S.~E. and {Douglas}, Kevin A. and {Korpela}, Eric J. and {Putman}, M.~E. and {Stanimirovi{\'c}}, Sne{\v{z}}ana and {Gibson}, Steven J. and {Heiles}, Carl},
        title = "{The GALFA-H I Survey Data Release 2}",
      journal = {\apjs},
     keywords = {methods: data analysis, radio lines: ISM, surveys},
         year = 2018,
        month = jan,
       volume = {234},
       number = {1},
          eid = {2},
        pages = {2},
          doi = {10.3847/1538-4365/aa91d3},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..234....2P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJS..194...20P,
       author = {{Peek}, J.~E.~G. and {Heiles}, Carl and {Douglas}, Kevin A. and {Lee}, Min-Young and {Grcevich}, Jana and {Stanimirovi{\'c}}, Sne{\v{z}}ana and {Putman}, M.~E. and {Korpela}, Eric J. and {Gibson}, Steven J. and {Begum}, Ayesha and {Saul}, Destry and {Robishaw}, Timothy and {Kr{\v{c}}o}, Marko},
        title = "{The GALFA-HI Survey: Data Release 1}",
      journal = {\apjs},
     keywords = {ISM: general, methods: data analysis, methods: observational, radio lines: ISM, surveys, techniques: imaging spectroscopy, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2011",
        month = jun,
       volume = {194},
       number = {2},
          eid = {20},
        pages = {20},
          doi = {10.1088/0067-0049/194/2/20},
archivePrefix = {arXiv},
       eprint = {1101.1879},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJS..194...20P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...539..273C,
       author = {{Cho}, Jungyeon and {Vishniac}, Ethan T.},
        title = "{The Anisotropy of Magnetohydrodynamic Alfv{\'e}nic Turbulence}",
      journal = {\apj},
     keywords = {ISM: General, Magnetic Fields, Magnetohydrodynamics: MHD, Turbulence, Astrophysics},
         year = 2000,
        month = aug,
       volume = {539},
       number = {1},
        pages = {273-282},
          doi = {10.1086/309213},
archivePrefix = {arXiv},
       eprint = {astro-ph/0003403},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...539..273C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020ApJ...898...66Y,
       author = {{Yuen}, Ka Ho and {Lazarian}, Alex},
        title = "{Curvature of Magnetic Field Lines in Compressible Magnetized Turbulence: Statistics, Magnetization Predictions, Gradient Curvature, Modes, and Self-gravitating Media}",
      journal = {\apj},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jul,
       volume = {898},
       number = {1},
          eid = {66},
        pages = {66},
          doi = {10.3847/1538-4357/ab9360},
archivePrefix = {arXiv},
       eprint = {2002.01926},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...898...66Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006ApJ...645L..25L,
       author = {{Lazarian}, A.},
        title = "{Enhancement and Suppression of Heat Transfer by MHD Turbulence}",
      journal = {\apjl},
     keywords = {Galaxies: Clusters: General, ISM: General, Magnetohydrodynamics: MHD, Turbulence, Astrophysics},
         year = 2006,
        month = jul,
       volume = {645},
       number = {1},
        pages = {L25-L28},
          doi = {10.1086/505796},
archivePrefix = {arXiv},
       eprint = {astro-ph/0608045},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...645L..25L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007JQSRT.106..225L,
       author = {{Lazarian}, A.},
        title = "{Tracing magnetic fields with aligned grains}",
      journal = {\jqsrt},
     keywords = {cosmic dust, interstellar dust, interstellar magnetic field, interstellar medium, polarimetry, stellar light polarisation, Astrophysics},
         year = 2007,
        month = jul,
       volume = {106},
        pages = {225-256},
          doi = {10.1016/j.jqsrt.2007.01.038},
archivePrefix = {arXiv},
       eprint = {0707.0858},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007JQSRT.106..225L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.457.2675H,
       author = {{Henshaw}, J.~D. and {Longmore}, S.~N. and {Kruijssen}, J.~M.~D. and {Davies}, B. and {Bally}, J. and {Barnes}, A. and {Battersby}, C. and {Burton}, M. and {Cunningham}, M.~R. and {Dale}, J.~E. and {Ginsburg}, A. and {Immer}, K. and {Jones}, P.~A. and {Kendrew}, S. and {Mills}, E.~A.~C. and {Molinari}, S. and {Moore}, T.~J.~T. and {Ott}, J. and {Pillai}, T. and {Rathborne}, J. and {Schilke}, P. and {Schmiedeke}, A. and {Testi}, L. and {Walker}, D. and {Walsh}, A. and {Zhang}, Q.},
        title = "{Molecular gas kinematics within the central 250 pc of the Milky Way}",
      journal = {\mnras},
     keywords = {stars: formation, ISM: clouds, ISM: kinematics and dynamics, ISM: structure, Galaxy: centre, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = apr,
       volume = {457},
       number = {3},
        pages = {2675-2702},
          doi = {10.1093/mnras/stw121},
archivePrefix = {arXiv},
       eprint = {1601.03732},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.457.2675H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019MNRAS.485.2457H,
       author = {{Henshaw}, J.~D. and {Ginsburg}, A. and {Haworth}, T.~J. and {Longmore}, S.~N. and {Kruijssen}, J.~M.~D. and {Mills}, E.~A.~C. and {Sokolov}, V. and {Walker}, D.~L. and {Barnes}, A.~T. and {Contreras}, Y. and {Bally}, J. and {Battersby}, C. and {Beuther}, H. and {Butterfield}, N. and {Dale}, J.~E. and {Henning}, T. and {Jackson}, J.~M. and {Kauffmann}, J. and {Pillai}, T. and {Ragan}, S. and {Riener}, M. and {Zhang}, Q.},
        title = "{`The Brick' is not a brick: a comprehensive study of the structure and dynamics of the central molecular zone cloud G0.253+0.016}",
      journal = {\mnras},
     keywords = {turbulence, stars: formation, ISM: clouds, ISM: kinematics and dynamics, ISM: structure, galaxy: centre, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = may,
       volume = {485},
       number = {2},
        pages = {2457-2485},
          doi = {10.1093/mnras/stz471},
archivePrefix = {arXiv},
       eprint = {1902.02793},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.485.2457H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.418..664N,
       author = {{Narayanan}, Desika and {Krumholz}, Mark and {Ostriker}, Eve C. and {Hernquist}, Lars},
        title = "{The CO-H$_{2}$ conversion factor in disc galaxies and mergers}",
      journal = {\mnras},
     keywords = {ISM: clouds, ISM: molecules, galaxies: interactions, galaxies: ISM, galaxies: starburst, galaxies: star formation, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2011,
        month = nov,
       volume = {418},
       number = {1},
        pages = {664-679},
          doi = {10.1111/j.1365-2966.2011.19516.x},
archivePrefix = {arXiv},
       eprint = {1104.4118},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.418..664N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016A&A...594A..25P,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Alves}, M.~I.~R. and {Arnaud}, M. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartlett}, J.~G. and {Bartolo}, N. and {Battaner}, E. and {Benabed}, K. and {Beno{\^\i}t}, A. and {Benoit-L{\'e}vy}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bonaldi}, A. and {Bonavera}, L. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Catalano}, A. and {Challinor}, A. and {Chamballu}, A. and {Chary}, R. -R. and {Chiang}, H.~C. and {Christensen}, P.~R. and {Colombi}, S. and {Colombo}, L.~P.~L. and {Combet}, C. and {Couchot}, F. and {Coulais}, A. and {Crill}, B.~P. and {Curto}, A. and {Cuttaia}, F. and {Danese}, L. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {D{\'e}sert}, F. -X. and {Dickinson}, C. and {Diego}, J.~M. and {Dole}, H. and {Donzelli}, S. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Falgarone}, E. and {Fergusson}, J. and {Finelli}, F. and {Forni}, O. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frejsel}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {Ghosh}, T. and {Giard}, M. and {Giraud-H{\'e}raud}, Y. and {Gjerl{\o}w}, E. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gregorio}, A. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Hansen}, F.~K. and {Hanson}, D. and {Harrison}, D.~L. and {Helou}, G. and {Henrot-Versill{\'e}}, S. and {Hern{\'a}ndez-Monteagudo}, C. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Hovest}, W. and {Huffenberger}, K.~M. and {Hurier}, G. and {Jaffe}, A.~H. and {Jaffe}, T.~R. and {Jones}, W.~C. and {Juvela}, M. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kisner}, T.~S. and {Kneissl}, R. and {Knoche}, J. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {L{\"a}hteenm{\"a}ki}, A. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Leahy}, J.~P. and {Leonardi}, R. and {Lesgourgues}, J. and {Levrier}, F. and {Liguori}, M. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Maris}, M. and {Marshall}, D.~J. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Matarrese}, S. and {McGehee}, P. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Mendes}, L. and {Mennella}, A. and {Migliaccio}, M. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Mortlock}, D. and {Moss}, A. and {Munshi}, D. and {Murphy}, J.~A. and {Nati}, F. and {Natoli}, P. and {Netterfield}, C.~B. and {N{\o}rgaard-Nielsen}, H.~U. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {Orlando}, E. and {Oxborrow}, C.~A. and {Paci}, F. and {Pagano}, L. and {Pajot}, F. and {Paladini}, R. and {Paoletti}, D. and {Partridge}, B. and {Pasian}, F. and {Patanchon}, G. and {Pearson}, T.~J. and {Peel}, M. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Piat}, M. and {Pierpaoli}, E. and {Pietrobon}, D. and {Plaszczynski}, S. and {Pointecouteau}, E. and {Polenta}, G. and {Pratt}, G.~W. and {Pr{\'e}zeau}, G. and {Prunet}, S. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reach}, W.~T. and {Rebolo}, R. and {Reinecke}, M. and {Remazeilles}, M. and {Renault}, C. and {Renzi}, A. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Rossetti}, M. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Rusholme}, B. and {Sandri}, M. and {Santos}, D. and {Savelainen}, M. and {Savini}, G. and {Scott}, D. and {Seiffert}, M.~D. and {Shellard}, E.~P.~S. and {Spencer}, L.~D. and {Stolyarov}, V. and {Stompor}, R. and {Strong}, A.~W. and {Sudiwala}, R. and {Sunyaev}, R. and {Sutton}, D. and {Suur-Uski}, A. -S. and {Sygnet}, J. -F. and {Tauber}, J.~A. and {Terenzi}, L. and {Toffolatti}, L. and {Tomasi}, M. and {Tristram}, M. and {Tucci}, M. and {Tuovinen}, J. and {Umana}, G. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, F. and {Vidal}, M. and {Vielva}, P. and {Villa}, F. and {Wade}, L.~A. and {Wandelt}, B.~D. and {Watson}, R. and {Wehus}, I.~K. and {Wilkinson}, A. and {Yvon}, D. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2015 results. XXV. Diffuse low-frequency Galactic foregrounds}",
      journal = {\aap},
     keywords = {diffuse radiation, ISM: general, radiation mechanisms: general, radio continuum: ISM, polarization, local insterstellar matter, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = sep,
       volume = {594},
          eid = {A25},
        pages = {A25},
          doi = {10.1051/0004-6361/201526803},
archivePrefix = {arXiv},
       eprint = {1506.06660},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...594A..25P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2012ApJS..200...20C,
       author = {{Clemens}, Dan P. and {Pinnick}, A.~F. and {Pavel}, M.~D.},
        title = "{Polarimetric Calibration of Mimir and the Galactic Plane Infrared Polarization Survey (GPIPS)}",
      journal = {\apjs},
     keywords = {Galaxy: disk, ISM: magnetic fields, magnetic fields, polarization, surveys, techniques: polarimetric},
         year = "2012",
        month = jun,
       volume = {200},
       number = {2},
          eid = {20},
        pages = {20},
          doi = {10.1088/0067-0049/200/2/20},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJS..200...20C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJS..200...21C,
       author = {{Clemens}, Dan P. and {Pavel}, M.~D. and {Cashman}, L.~R.},
        title = "{The Galactic Plane Infrared Polarization Survey (GPIPS): Data Release 1}",
      journal = {\apjs},
     keywords = {Galaxy: disk, ISM: magnetic fields, magnetic fields, polarization, surveys, techniques: polarimetric},
         year = "2012",
        month = jun,
       volume = {200},
       number = {2},
          eid = {21},
        pages = {21},
          doi = {10.1088/0067-0049/200/2/21},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJS..200...21C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2013AAS...22135215C,
       author = {{Clemens}, Dan P. and {Cashman}, L.~R. and {Hoq}, S. and {Montgomery}, J. and {Pavel}, M.~D.},
        title = "{The Galactic Plane Infrared Polarization Survey (GPIPS): The Full Poster}",
    booktitle = {American Astronomical Society Meeting Abstracts \#221},
         year = 2013,
       series = {American Astronomical Society Meeting Abstracts},
       volume = {221},
        month = jan,
          eid = {352.15},
        pages = {352.15},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013AAS...22135215C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2018ApJ...868L..33L,
       author = {{Li}, Leping and {Zhang}, Jun and {Peter}, Hardi and
         {Chitta}, Lakshmi Pradeep and {Su}, Jiangtao and {Song}, Hongqiang and
         {Xia}, Chun and {Hou}, Yijun},
        title = "{Quasi-periodic Fast Propagating Magnetoacoustic Waves during the Magnetic Reconnection Between Solar Coronal Loops}",
      journal = {\apj},
     keywords = {magnetic reconnection, plasmas, Sun: corona, Sun: UV radiation, waves, Astrophysics - Solar and Stellar Astrophysics},
         year = "2018",
        month = "Dec",
       volume = {868},
       number = {2},
          eid = {L33},
        pages = {L33},
          doi = {10.3847/2041-8213/aaf167},
archivePrefix = {arXiv},
       eprint = {1811.08553},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...868L..33L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016AJ....152...41P,
       author = {{Pr{\v{s}}a}, Andrej and {Harmanec}, Petr and {Torres}, Guillermo and
         {Mamajek}, Eric and {Asplund}, Martin and {Capitaine}, Nicole and
         {Christensen-Dalsgaard}, J{\o}rgen and {Depagne}, {\'E}ric and
         {Haberreiter}, Margit and {Hekker}, Saskia},
        title = "{Nominal Values for Selected Solar and Planetary Quantities: IAU 2015 Resolution B3}",
      journal = {\aj},
     keywords = {planets and satellites: fundamental parameters, standards, stars: fundamental parameters, stars: general, Sun: fundamental parameters, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2016",
        month = "Aug",
       volume = {152},
       number = {2},
          eid = {41},
        pages = {41},
          doi = {10.3847/0004-6256/152/2/41},
archivePrefix = {arXiv},
       eprint = {1605.09788},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016AJ....152...41P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ApJ...517..700L,
       author = {{Lazarian}, A. and {Vishniac}, Ethan T.},
        title = "{Reconnection in a Weakly Stochastic Field}",
      journal = {\apj},
     keywords = {GALAXIES: MAGNETIC FIELDS, MAGNETOHYDRODYNAMICS: MHD, Galaxies: Magnetic Fields, Magnetohydrodynamics: MHD, Astrophysics, Physics - Fluid Dynamics, Physics - Geophysics, Physics - Plasma Physics, Physics - Space Physics},
         year = 1999,
        month = jun,
       volume = {517},
       number = {2},
        pages = {700-718},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...517..700L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2007AGUFMSH32B..02L,
       author = {{Lazarian}, A.},
        title = "{Properties of Compressible MHD Turbulence}",
     keywords = {2104 Cosmic rays, 2114 Energetic particles (7514), 2126 Heliosphere/interstellar medium interactions, 2149 MHD waves and turbulence (2752, 6050, 7836), 2159 Plasma waves and turbulence},
    booktitle = {AGU Fall Meeting Abstracts},
         year = 2007,
       volume = {2007},
        month = dec,
          eid = {SH32B-02},
        pages = {SH32B-02},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007AGUFMSH32B..02L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJS..197...31S,
       author = {{Schwarz}, Greg J. and {Ness}, Jan-Uwe and {Osborne}, J.~P. and
         {Page}, K.~L. and {Evans}, P.~A. and {Beardmore}, A.~P. and
         {Walter}, Frederick M. and {Helton}, L. Andrew and
         {Woodward}, Charles E. and {Bode}, Mike and {Starrfield}, Sumner and
         {Drake}, Jeremy J.},
        title = "{Swift X-Ray Observations of Classical Novae. II. The Super Soft Source Sample}",
      journal = {\apjs},
     keywords = {novae, cataclysmic variables, ultraviolet: stars, X-rays: stars, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2011",
        month = "Dec",
       volume = {197},
       number = {2},
          eid = {31},
        pages = {31},
          doi = {10.1088/0067-0049/197/2/31},
archivePrefix = {arXiv},
       eprint = {1110.6224},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJS..197...31S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000AJ....119..923H,
       author = {{Heiles}, Carl},
        title = "{9286 Stars: An Agglomeration of Stellar Polarization Catalogs}",
      journal = {\aj},
     keywords = {CATALOGS, ISM: DUST, EXTINCTION, ISM: MAGNETIC FIELDS, STARS: DISTANCES, Astrophysics},
         year = 2000,
        month = feb,
       volume = {119},
       number = {2},
        pages = {923-927},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000AJ....119..923H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

 @ARTICLE{1978MNRAS.182..147B,
       author = {{Bell}, A.~R.},
        title = "{The acceleration of cosmic rays in shock fronts - I.}",
      journal = {\mnras},
     keywords = {Cosmic Rays, Particle Acceleration, Relativistic Particles, Shock Fronts, Electrostatic Waves, Energy Spectra, Galactic Radiation, Magnetohydrodynamic Waves, Oblique Shock Waves, Shock Wave Propagation, Space Radiation, Cosmic Rays:Energy Spectra, Cosmic Rays:Galaxy, Cosmic Rays:Shock Waves},
         year = 1978,
        month = jan,
       volume = {182},
        pages = {147-156},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1978MNRAS.182..147B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1966ApJ...146..480J,
       author = {{Jokipii}, J.~R.},
        title = "{Cosmic-Ray Propagation. I. Charged Particles in a Random Magnetic Field}",
      journal = {\apj},
         year = 1966,
        month = nov,
       volume = {146},
        pages = {480},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1966ApJ...146..480J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004RvMP...76..125M,
       author = {{Mac Low}, Mordecai-Mark and {Klessen}, Ralf S.},
        title = "{Control of star formation by supersonic turbulence}",
      journal = {Reviews of Modern Physics},
     keywords = {97.10.Bt, 98.62.Ai, 95.30.Lz, 95.30.Sf, 47.27.-i, 47.40.Ki, Star formation, Origin formation evolution age and star formation, Hydrodynamics, Relativity and gravitation, Turbulent flows, Supersonic and hypersonic flows, Astrophysics},
         year = 2004,
        month = jan,
       volume = {76},
       number = {1},
        pages = {125-194},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004RvMP...76..125M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...793..127V,
       author = {{Vogt}, Fr{\'e}d{\'e}ric P.~A. and {Dopita}, Michael A. and
         {Kewley}, Lisa J. and {Sutherland}, Ralph S. and
         {Scharw{\"a}chter}, Julia and {Basurah}, Hassan M. and {Ali}, Alaa and
         {Amer}, Morsi A.},
        title = "{Galaxy Emission Line Classification Using Three-dimensional Line Ratio Diagrams}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: general, galaxies: Seyfert, galaxies: starburst, H II regions, ISM: lines and bands, Astrophysics - Astrophysics of Galaxies},
         year = "2014",
        month = "Oct",
       volume = {793},
       number = {2},
          eid = {127},
        pages = {127},
          doi = {10.1088/0004-637X/793/2/127},
archivePrefix = {arXiv},
       eprint = {1406.5186},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...793..127V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ARA&A..45..565M,
       author = {{McKee}, Christopher F. and {Ostriker}, Eve C.},
        title = "{Theory of Star Formation}",
      journal = {\araa},
     keywords = {Astrophysics},
         year = 2007,
        month = sep,
       volume = {45},
       number = {1},
        pages = {565-687},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ARA&A..45..565M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ARA&A..42..211E,
       author = {{Elmegreen}, Bruce G. and {Scalo}, John},
        title = "{Interstellar Turbulence I: Observations and Processes}",
      journal = {\araa},
     keywords = {Astrophysics},
         year = 2004,
        month = sep,
       volume = {42},
       number = {1},
        pages = {211-273},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ARA&A..42..211E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995ApJ...438..763G,
       author = {{Goldreich}, P. and {Sridhar}, S.},
        title = "{Toward a Theory of Interstellar Turbulence. II. Strong Alfvenic Turbulence}",
      journal = {\apj},
     keywords = {Interstellar Space, Magnetic Fields, Magnetohydrodynamic Turbulence, Magnetohydrodynamic Waves, Electron Density (Concentration), Energy Spectra, Radio Waves, Variations, Wave Scattering, Astrophysics, ISM: GENERAL, MAGNETOHYDRODYNAMICS: MHD, TURBULENCE},
         year = 1995,
        month = jan,
       volume = {438},
        pages = {763},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...438..763G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...783...91C,
       author = {{Caprioli}, D. and {Spitkovsky}, A.},
        title = "{Simulations of Ion Acceleration at Non-relativistic Shocks. I. Acceleration Efficiency}",
      journal = {\apj},
     keywords = {acceleration of particles, ISM: supernova remnants, magnetic fields, shock waves, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = mar,
       volume = {783},
       number = {2},
          eid = {91},
        pages = {91},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...783...91C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017ApJ...835...41G,
       author = {{Gonz{\'a}lez-Casanova}, Diego F. and {Lazarian}, A.},
        title = "{Velocity Gradients as a Tracer for Magnetic Fields}",
      journal = {\apj},
     keywords = {ISM: kinematics and dynamics, ISM: magnetic fields, magnetohydrodynamics: MHD, turbulence, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jan,
       volume = {835},
       number = {1},
          eid = {41},
        pages = {41},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...835...41G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1956MNRAS.116..503M,
       author = {{Mestel}, L. and {Spitzer}, L., Jr.},
        title = "{Star formation in magnetic dust clouds}",
      journal = {\mnras},
         year = 1956,
        month = jan,
       volume = {116},
        pages = {503},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1956MNRAS.116..503M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020A&A...641A..12P,
       author = {{Planck Collaboration} and {Aghanim}, N. and {Akrami}, Y. and {Alves}, M.~I.~R. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basak}, S. and {Benabed}, K. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bock}, J.~J. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bracco}, A. and {Bucher}, M. and {Burigana}, C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Carron}, J. and {Chary}, R. -R. and {Chiang}, H.~C. and {Colombo}, L.~P.~L. and {Combet}, C. and {Crill}, B.~P. and {Cuttaia}, F. and {de Bernardis}, P. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {Di Valentino}, E. and {Dickinson}, C. and {Diego}, J.~M. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dupac}, X. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Falgarone}, E. and {Fantaye}, Y. and {Fernandez-Cobos}, R. and {Ferri{\`e}re}, K. and {Finelli}, F. and {Forastieri}, F. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and {Ghosh}, T. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Green}, G. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Guillet}, V. and {Handley}, W. and {Hansen}, F.~K. and {Helou}, G. and {Herranz}, D. and {Hivon}, E. and {Huang}, Z. and {Jaffe}, A.~H. and {Jones}, W.~C. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kiiveri}, K. and {Kim}, J. and {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Levrier}, F. and {Liguori}, M. and {Lilje}, P.~B. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marcos-Caballero}, A. and {Maris}, M. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {Mauri}, N. and {McEwen}, J.~D. and {Melchiorri}, A. and {Mennella}, A. and {Migliaccio}, M. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Moss}, A. and {Natoli}, P. and {Pagano}, L. and {Paoletti}, D. and {Patanchon}, G. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Polastri}, L. and {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Ristorcelli}, I. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Salvati}, L. and {Sandri}, M. and {Savelainen}, M. and {Scott}, D. and {Sirignano}, C. and {Sunyaev}, R. and {Suur-Uski}, A. -S. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Tenti}, M. and {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and {Valiviita}, J. and {Vansyngel}, F. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2018 results. XII. Galactic astrophysics using polarized dust emission}",
      journal = {\aap},
     keywords = {polarization, magnetic fields, turbulence, dust, extinction, local insterstellar matter, submillimeter: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2020",
        month = sep,
       volume = {641},
          eid = {A12},
        pages = {A12},
          doi = {10.1051/0004-6361/201833885},
archivePrefix = {arXiv},
       eprint = {1807.06212},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A..12P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1959ApJ...129..243S,
       author = {{Schmidt}, Maarten},
        title = "{The Rate of Star Formation.}",
      journal = {\apj},
         year = 1959,
        month = mar,
       volume = {129},
        pages = {243},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1959ApJ...129..243S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018MNRAS.480.1333H,
       author = {{Hu}, Yue and {Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Improving the accuracy of magnetic field tracing by velocity gradients: principal component analysis}",
      journal = {\mnras},
     keywords = {magnetohydrodynamics (MHD), turbulence, methods: numerical, ISM: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = oct,
       volume = {480},
       number = {1},
        pages = {1333-1339},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.480.1333H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019ApJ...872...56P,
       author = {{Panopoulou}, Georgia V. and {Tassis}, Konstantinos and {Skalidis}, Raphael and {Blinov}, Dmitriy and {Liodakis}, Ioannis and {Pavlidou}, Vasiliki and {Potter}, Stephen B. and {Ramaprakash}, Anamparambu N. and {Readhead}, Anthony C.~S. and {Wehus}, Ingunn K.},
        title = "{Demonstration of Magnetic Field Tomography with Starlight Polarization toward a Diffuse Sightline of the ISM}",
      journal = {\apj},
     keywords = {ISM: clouds, ISM: magnetic fields, techniques: polarimetric, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = feb,
       volume = {872},
       number = {1},
          eid = {56},
        pages = {56},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...872...56P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019ApJ...886...17H,
       author = {{Hu}, Yue and {Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Intensity Gradients Technique: Synergy with Velocity Gradients and Polarization Studies}",
      journal = {\apj},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = nov,
       volume = {886},
       number = {1},
          eid = {17},
        pages = {17},
          doi = {10.3847/1538-4357/ab4b5e},
archivePrefix = {arXiv},
       eprint = {1908.09488},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...886...17H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021ApJ...912....2H,
       author = {{Hu}, Yue and {Lazarian}, A. and {Stanimirovi{\'c}}, Sne{\v{z}}ana},
        title = "{Revealing Gravitational Collapse in the Serpens G3-G6 Molecular Cloud Using Velocity Gradients}",
      journal = {\apj},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, Star-forming regions, 847, 845, 839, 1565, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
       volume = {912},
       number = {1},
          eid = {2},
        pages = {2},
          doi = {10.3847/1538-4357/abedb7},
archivePrefix = {arXiv},
       eprint = {2102.06225},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...912....2H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020ApJ...901..162H,
       author = {{Hu}, Yue and {Lazarian}, A. and {Li}, Yuan and {Zhuravleva}, Irina and {Gendron-Marsolais}, Marie-Lou},
        title = "{Probing Magnetic Field Morphology in Galaxy Clusters with the Gradient Technique}",
      journal = {\apj},
     keywords = {Intracluster medium, Extragalactic magnetic fields, Magnetohydrodynamics, Galaxy clusters, 858, 507, 1964, 584, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = oct,
       volume = {901},
       number = {2},
          eid = {162},
        pages = {162},
          doi = {10.3847/1538-4357/abb1c3},
archivePrefix = {arXiv},
       eprint = {2007.06219},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...901..162H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995ApJ...443..209A,
       author = {{Armstrong}, J.~W. and {Rickett}, B.~J. and {Spangler}, S.~R.},
        title = "{Electron Density Power Spectrum in the Local Interstellar Medium}",
      journal = {\apj},
     keywords = {Electron Density Profiles, Interstellar Matter, Power Spectra, Scintillation, Astronomical Models, Plasma Turbulence, Pulsars, Radio Astronomy, Astrophysics, ISM: STRUCTURE, RADIO CONTINUUM: ISM, STARS: PULSARS: GENERAL, TURBULENCE},
         year = 1995,
        month = apr,
       volume = {443},
        pages = {209},
          doi = {10.1086/175515},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...443..209A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1981MNRAS.194..809L,
       author = {{Larson}, R.~B.},
        title = "{Turbulence and star formation in molecular clouds.}",
      journal = {\mnras},
     keywords = {Interstellar Matter, Molecular Clouds, Protostars, Star Formation, Turbulence Effects, Clumps, Density Distribution, Stellar Gravitation, Stellar Mass, Velocity Distribution, Virial Theorem, Astrophysics},
         year = 1981,
        month = mar,
       volume = {194},
        pages = {809-826},
          doi = {10.1093/mnras/194.4.809},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1981MNRAS.194..809L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020ApJ...897..123H,
       author = {{Hu}, Yue and {Lazarian}, A. and {Yuen}, Ka Ho},
        title = "{Velocity Gradient in the Presence of Self-gravity: Identifying Gravity-induced Inflow and Determining Collapsing Stage}",
      journal = {\apj},
     keywords = {845, 1569, 847, 1565, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = jul,
       volume = {897},
       number = {2},
          eid = {123},
        pages = {123},
          doi = {10.3847/1538-4357/ab9948},
archivePrefix = {arXiv},
       eprint = {2002.06754},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...897..123H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020PhPl...27a2305L,
       author = {{Lazarian}, Alex and {Eyink}, Gregory L. and {Jafari}, Amir and {Kowal}, Grzegorz and {Li}, Hui and {Xu}, Siyao and {Vishniac}, Ethan T.},
        title = "{3D turbulent reconnection: Theory, tests, and astrophysical implications}",
      journal = {Physics of Plasmas},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Physics - Computational Physics, Physics - Plasma Physics},
         year = 2020,
        month = jan,
       volume = {27},
       number = {1},
          eid = {012305},
        pages = {012305},
          doi = {10.1063/1.5110603},
archivePrefix = {arXiv},
       eprint = {2001.00868},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020PhPl...27a2305L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ApJ...865...59L,
       author = {{Lazarian}, A. and {Yuen}, Ka Ho},
        title = "{Gradients of Synchrotron Polarization: Tracing 3D Distribution of Magnetic Fields}",
      journal = {\apj},
     keywords = {ISM: general, ISM: magnetic fields, ISM: structure, magnetohydrodynamics: MHD, radio continuum: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2018a",
        month = sep,
       volume = {865},
       number = {1},
          eid = {59},
        pages = {59},
          doi = {10.3847/1538-4357/aad3ca},
archivePrefix = {arXiv},
       eprint = {1802.00028},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...865...59L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ApJ...855...72L,
       author = {{Lazarian}, A. and {Yuen}, Ka Ho and {Lee}, Hyeseung and {Cho}, J.},
        title = "{Erratum: {\textquotedblleft}Synchrotron Intensity Gradients as Tracers of Interstellar Magnetic Fields{\textquotedblright} (<A href=``http://doi.org/10.3847/1538-4357/aa74c6''>2017, ApJ, 842, 1, 30</A>)}",
      journal = {\apj},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = mar,
       volume = {855},
       number = {1},
          eid = {72},
        pages = {72},
          doi = {10.3847/1538-4357/aaae02},
archivePrefix = {arXiv},
       eprint = {1701.07883},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...855...72L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021arXiv211115066H,
       author = {{Hu}, Yue and {Lazarian}, A. and {Xu}, Siyao},
        title = "{Superdiffusion of Cosmic Rays in Compressible Magnetized Turbulence}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = nov,
          eid = {arXiv:2111.15066},
        pages = {arXiv:2111.15066},
archivePrefix = {arXiv},
       eprint = {2111.15066},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv211115066H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


